Gradient-Variation Online Learning under Generalized Smoothness

Gradient-variation online learning aims to achieve regret guarantees that scale with variations in the gradients of online functions, which has been shown to be crucial for attaining fast convergence in games and robustness in stochastic optimization, hence receiving increased attention. Existing results often require the smoothness condition by imposing a fixed bound on gradient Lipschitzness, which may be unrealistic in practice. Recent efforts in neural network optimization suggest a generalized smoothness condition, allowing smoothness to correlate with gradient norms. In this paper, we systematically study gradient-variation online learning under generalized smoothness. We extend the classic optimistic mirror descent algorithm to derive gradient-variation regret by analyzing stability over the optimization trajectory and exploiting smoothness locally. Then, we explore universal online learning, designing a single algorithm with the optimal gradient-variation regrets for convex and strongly convex functions simultaneously, without requiring prior knowledge of curvature. This algorithm adopts a two-layer structure with a meta-algorithm running over a group of base-learners. To ensure favorable guarantees, we design a new Lipschitz-adaptive meta-algorithm, capable of handling potentially unbounded gradients while ensuring a second-order bound to effectively ensemble the base-learners. Finally, we provide the applications for fast-rate convergence in games and stochastic extended adversarial optimization.

==> sections/extensions.tex <==
%!TEX root = ../nips24_local-smooth_vCRC.tex
\section{Extensions}
\label{sec:extensions}
We extend our algorithm to scenario where much uncertainty should be considered to ensure robust results.
\subsection{Extension to Dynamic Regret Minimization}
\begin{itemize}
  \item First dynamic regret bound with gradient-variation bound under generalized smoothness. Since the Lipschitzness of gradients are unknown in previous, the base-learners should make self-confident tuning.
  \item Compared to~\citet{NIPS'20:sword}, our base-leaner are similar, but we use function value to derive the gradient-variation bound due to the technique~\citet{arxiv23:omd4sea, NeurIPS'22:label_shift} in the meta level, failed to imply the best-of-both-worlds bounds. However, by applying \textsc{MsMwC}~\citep{COLT'21:impossible-tuning} as the meta-learner and the techniques used in~\citet{NIPS'20:sword}, we can achieve the best-of-both-worlds results will suffering additional $\O(\sqrt{\log T})$ terms.
  \item Compared to Sword++~\citet{JMLR:sword++}, we queries $\O(3\log T)$ times of gradients per round, since we need local approximation and one gradient seems not enough to ensure the local smoothness.
\end{itemize}
\subsection{Extension to Adaptive Regret Minimization}
\begin{itemize}
  \item The fixed point solution is in one dimension, and thus it is not computationally dominated.
  \item The first adaptive regret in gradient variation while agnostic to the smoothness in previous.
  \item Still unknown how to achieve the fully-problem dependent bound.
\end{itemize}
\subsection{Extension to Unbounded Domain}
\begin{itemize}
  \item Similar structure to the one for obtaining dynamic regret. Indeed inspired by~\citet{COLT'22:Corral++}, we can build the grid and obtain the bound adaptive to both the unbounded domain and arbitrary comparators.
  \item Employ $\O(T)$ learners can compare to $\Ot(\norm{\u})$, and employ $\O(\log (T))$ experts can compare to $\O(\norm{\u}^2)$.
\end{itemize}
